NanoFlow: Towards Optimal Large Language Model Serving Throughput

Large Language Models (LLMs) have resulted in a surging demand for planet-scale serving systems, where tens of thousands of GPUs continuously serve hundreds of millions of users. Consequently, throughput has emerged as a key metric that determines serving systems' performance. Due to large model sizes and memory-intensive self-attention, LLM serving has been commonly assumed to be memory-bound. Through a detailed analysis, we show that despite having memory-intensive components, end-to-end LLM serving is compute bound for most common workloads and LLMs. Alas, most existing serving engines fall short from optimal compute utilization, because the heterogeneous operations that comprise LLM serving--compute, memory, networking--are executed sequentially within a device. We propose NanoFlow, a novel serving framework that exploits intra-device parallelism, which overlaps the usage of heterogeneous resources within a single device. NanoFlow splits inputs into smaller nano-batches and duplicates operations to operate on each portion independently, enabling overlapping. NanoFlow automatically identifies the number, size, ordering, and GPU resource allocation of nano-batches to minimize the execution time, while considering the interference of concurrent operations. We evaluate NanoFlow's end-to-end serving throughput on several popular models such as LLaMA-2-70B, Mixtral 8x7B, LLaMA-3-8B, etc. With practical workloads, NanoFlow provides 1.91x throughput boost compared to state-of-the-art serving systems achieving 50% to 72% of optimal throughput across popular models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.03.  Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples <==
% Teach biblatex about numpages field
\DeclareDatamodelFields[type=field, datatype=literal]{numpages}
\DeclareDatamodelEntryfields{numpages}

% Teach biblatex about articleno field
\DeclareDatamodelFields[type=field, datatype=literal]{articleno}
\DeclareDatamodelEntryfields{articleno}

% Teach biblatex about urls field
\DeclareDatamodelFields[type=list, datatype=uri]{urls}
\DeclareDatamodelEntryfields{urls}

% Teach biblatex about school field
\DeclareDatamodelFields[type=list, datatype=literal]{school}
\DeclareDatamodelEntryfields[thesis]{school}

\DeclareDatamodelFields[type=field, datatype=literal]{key}
\DeclareDatamodelEntryfields{key}

% Teach biblatex about lastaccessed field
\DeclareDatamodelFields[type=field,datatype=literal]{lastaccessed}
\DeclareDatamodelEntryfields{lastaccessed}

% Teach biblatex about distincturl field
\DeclareDatamodelFields[type=field, datatype=literal]{distinctURL}
\DeclareDatamodelEntryfields{distinctURL}


%
% include software data model from biblatex-software
%

\blx@inputonce{software.dbx}{biblatex data model extension for software}{}{}{}{}


==> src/01-2_Introduction.tex <==
\section{Introduction}
\label{sec:intro}

Large language models (LLMs) based on the transformer architecture power applications like chatbots, search engines, and office software but are highly resource-intensive~\cite{Mehdi_2023, Spataro_2023, ChatGPT}. Reports indicate over $200$ million weekly ChatGPT users, with API usage doubling after GPT-4o Mini's release~\cite{seminanalysis,demandsageChatGPTStatistics,openai_chatgpt_verge}. Given the massive demand and limited GPU availability~\cite{gpushortage, nytgpushortage}, maximizing hardware utilization is critical. In particular, throughput, measured as tokens per device per second, has become a key factor in reducing serving costs~\cite{vllm, deepspeed-fastgen, tensorrtllm}.



LLMs are more resource-intensive than earlier DNNs due to unique characteristics. Their model sizes are vastly larger, such as GPT-3 with 175B parameters requiring $5\times$A100 GPUs to store weights, with some closed-source models even larger~\cite{brown2020language}. Moreover, LLMs' self-attention mechanism~\cite{attention} scales memory usage linearly with context length---the aggregate length of input and output sequences---during token generation. LLM serving systems often cache per-request state in a \emph{key-value cache} (\kv{}), whose size can surpass the size of model weights~\cite{tang2024quest}, driving up memory demands.


Due to these characteristics, LLM serving is commonly assumed to be memory-bound. Consequently, a wide body of research has studied the memory behavior of LLM inference, and proposed techniques to optimize memory accesses~\cite{dao2023flashattention2} and reduce fragmentation~\cite{vllm}. Similarly, most popular serving frameworks\cite{vllm, deepspeed-fastgen, tensorrtllm} use large request batch sizes to amortize the weight loading cost.

In this paper, we first provide a detailed analytical analysis and empirical validation~(\S\ref{sec:analysis}), which shows that this conventional assumption obscures a critical insight: Under the current large GPU-level batch sizes commonly used in LLM serving, compute-bound operations increasingly dominate performance. Specifically, while operations such as decode attention and network communication remain memory and network bound, respectively, amortized weight loading shifts general matrix multiplication (GEMM) operations towards a compute-bound regime. Moreover, optimizations such as grouped query attention~\cite{ainslie2023gqa} (GQA) further reduce the memory intensity of workloads, by decreasing the capacity of the required \kv{}. Consequently, for a variety of user inputs and models, the time spent on compute-bound operations becomes the primary throughput bottleneck of LLM serving.



Our analysis reveals that the conventional practice of maintaining a single large batch at the GPU-level is limited in that it falls far from the optimal solution for throughput-oriented serving of modern LLMs. This is not helped by prior work's use of inter-device parallelism, which executes batches in parallel across GPUs\cite{alpa, megatron-lm,huang2019gpipe}. Consequently, these systems load a single large batch of requests into a GPU and process it sequentially through a transformer's layers, where each layer involves operations that are individually compute-, memory- and network- bound. We find that the sequential execution of these operations at the device-level leads to significant under-utilization of compute, the most constrained resource. \kan{how bad they are? characteristics?}
\arvind{Not sure whether the flow/logic of the previous two paras works. An alternate version could be as follows: (1) LLM serving is commonly believed to be memory bound. (2) We did an extensive empirical analysis and we found that this is actually a consequence of the execution model that processes a single large batch through different stages of the LLM. (3) We also find that, fundamentally, there is sufficient compute to amortize the memory costs and have the entire operation be compute-bound if the execution is structured appropriately. (In particular, I think it would be good to have the contrast between what others have assumed and what our findings are right next to each other. This makes it a "surprising" result.)}\baris{I don't think I quite get 2). "This" is not a consequence, since we find out it is not true. Do you mean "the belief" by "this"? If so, it'd be hard to deduce where the belief stems from. I think it is mostly because things started off without GQA and smaller models. There is a misconception, which we find out by looking at the operation characteristics.}\arvind{It might be good to chat about this, as there might be different ways to tell the story here. Here is my updated view: (1) Current understanding in the field -- prefill is compute bound (especially after flash attention), decode is memory bound. Systems try to reduce the memory-boundedness of decode by batching it with prefill, but overall execution still appears to be memory bound - as in, the arithmetic intensity is not high enough in practice. (2) Our analysis attempts to characterize the "fundamental" resource bottleneck in serving that is independent of how operations are scheduled. Note that compute-boundedness and memory-boundedness are a function of how operations are scheduled (as in before Flash-Attention, prefill attention was memory-bound and after FA, it became compute-bound). So we are asking what is the fundamental nature of the computation and we come up with a different viewpoint. (3) The gap between this fundamental nature and today's realized performance is how operations are scheduled. Heterogeneous resources are not used at the same time. Nanobatching lets us do that and as a consequence lets us distill an implementation that is actually compute-bound that matches the fundamental nature.}

To overcome the aforementioned limitation, we propose \pllm{}, a serving framework where we rethink batch processing during LLM serving. Specifically, we propose \textit{\nano{}ing}, which duplicates transformer operations and splits their inputs into finer-grained units called \textit{\nano{}es}. Each resulting operation, called a \textit{\nanoop{}}, processes a portion of the input independently. By breaking dependencies in this way, \nanoop{}s that are bound by hetereogeneous resources such as compute, memory, and networking, can execute in parallel within a device---intra-device paralellism---, significantly improving resource utilization.Our key insight is that, while \nano{}ing incurs additional model weight loading overhead, this cost is subsumed in compute-bound LLM serving due to the high-degree of parallelism it enables. \baris{Stephanie: this last sentence is obscure. explain better/get rid of.} 









Designing \pllm{} presents several major challenges. First, given the multitude and diversity of LLMs, determining the appropriate number of \nano{}es, the input batch size per each \nanoop{}, and the execution order of \nanoop{}s involves navigating a large search space. Second, when memory- or network-bound kernels run alongside compute-bound kernels, competition for GPU resources (e.g., execution units, caches) causes performance interference, slowing down kernels running in parallel. Balancing these trade-offs is critical. Allocating more resources to compute-bound kernels may excessively delay memory- or network-bound kernels, while prioritizing memory- or network-bound kernels could hinder overall throughput by slowing down compute-bound operations. 

To tackle these challenges and efficiently explore the large search space, \pllm{} automatically constructs an intra-device pipeline aimed at maximizing the parallel execution of \nanoop{}s by accounting for operation dependencies and kernel profiling results. Due to the complexity, this \textit{auto-search} process consists of two stages. In the first stage, \pllm{} determines the initial pipeline schedule, including the number, size, and ordering of \nanoop{}s, assuming no interference between kernels. In the second stage, \pllm{} refines the pipeline by optimizing GPU resource allocation to minimize kernel interference. \pllm{} assigns heterogeneous \nanoop{}s to heterogeneous resources on the GPU, where for instance, a compute-heavy operation can be scheduled to consume more resources (e.g., thread blocks) than a memory-bound operation, which could use the entire memory bandwidth with fewer resources. 



\pllm{} also provides a runtime system to execute the optimized pipeline by efficiently forming \nano{}es, allocating GPU resources, and managing the KV cache. \pllm{}'s runtime schedule prefill requests at a finer granularity than prior work~\cite{sarathi-serve} to maintain exact batch sizes chosen by its profiling to deliver the highest throughput and consistent latency, while respecting memory capacity constraints.
 \pllm{}'s runtime dynamically partitions GPU resources by launching the kernels determined by its \auto{}. Additionally, \pllm{} coalesces \kv{} pages and moves contiguous data between the CPU and GPU, in parallel with the pipeline execution. This approach supports multi-round conversations without costly recomputation.





















 



We provide a detailed evaluation of \pllm{} on the \lm{}-2-70B model~\cite{llama2} using one NVIDIA $8\times$A100 DGX node~\cite{dgx}. Under practical workloads collected from ShareGPT~\cite{sharegpt}, LMSys~\cite{zheng2023lmsyschat1m} and Splitwise~\cite{splitwise}, \pllm{} achieves on average \computesota{} greater throughput compared with state-of-the-art serving frameworks including vLLM \cite{vllm}, DeepSpeed-FastGen \cite{deepspeed-fastgen} and TensorRT-LLM \cite{tensorrtllm}, which is \computeoptimalratio{} of the theoretically optimal throughput we derive in \S\ref{sec:analysis}. \pllm{} achieves similar latency compared with the best baseline TensorRT-LLM at a low request rate, while handling up to \requestsota{} higher request rates within SLO constraint. We demonstrate \pllm{}'s ability to automatically generate efficient pipelines for other models and architectures (such as Mixture-of-Experts (MoE)), by evaluating popular LLMs (\lm{}-3-70B, \lm{}-3-8B, QWen2-72B, Deepseek-67B, and Mixtral 8$\times$7B). \pllm{}-generated serving pipelines achieve \portmin-\portmax of optimal throughput. \kan{measure again later}


In summary, we contribute the following:
\begin{itemize}[noitemsep, topsep=0pt]
    \item A detailed analysis and empirircal validation of the workload characteristics and theoretically optimal throughput of LLM serving systems that shows modern LLMs to operate in a compute-bound regime. 
    \item \pllm{}, that comprises (1) an auto-search engine that automatically computes a pipeline for \nano{}es to improve LLM serving throughput, (2) an end-to-end LLM serving runtime.
    \item A comprehensive evaluation of \pllm{} that achieves \computesota{} throughput gain compared to baselines and \computeoptimalratio{} of theoretical maximum throughput.
\end{itemize}




==> src/04_Design.tex <==
\section{Design}


We introduce \pllm{}'s key components: the \auto{} engine for automatic \nano{} pipeline computation (\S\ref{sec:design}) and the LLM serving runtime for pipeline execution (\S\ref{sec:implementation}).

\subsection{Automated Pipeline Search}
\label{sec:design}

Forming \nanoop{}s, launching kernels, and scheduling with \newparall{} is challenging due to model and hardware diversity. To address this, \pllm{} proposes \auto{}, \new{which uses mixed integer linear programming to obtain the \nano{} overlapping strategy, via a two-stage approximation for reducing search space}.
We first outline \auto{} prerequisites like kernel profiling and interference modeling (\S\ref{subsec:kernel-profile}), then detail its two stages: pipeline structure search (\S\ref{subsec: pipeline-search}) and GPU resource allocation (\S\ref{subsec: resource-search}). Finally, we provide example pipelines for popular models (\S\ref{subsec: case-study}).


\subsubsection{Kernel Profiling and Interference Modeling}
\label{subsec:kernel-profile}
Understanding the performance characteristics of different operations is key to automated pipeline search. For this, \pllm{} profiles GEMM kernels (used for compute-bound operations. E.g., KQV generation), GEMV kernels (used in memory-bound operations as in decode-attention) and network kernels (used in network-bound operations such as all reduce and all gather). 

\textbf{Determining the maximum dense batch size}
Given a specific model architecture and user input statistics (as described in \S\ref{sec:costfactors}), \pllm{} calculates the maximum dense batch size that can fit into the GPU memory (e.g. 2048 for $8\times A100$ serving Llama 70B). This dense batch size sets an upper bound in profiling and serves as an input to \auto{}.

\textbf{Profiling interference-free kernels}
\pllm{} then determines the interference-free execution time of kernels, where each operation exclusively uses the GPU. \pllm{} profiles kernels with discrete batch sizes from 128 to the dense batch size in multiples of 128. \new{This also increases hardware utilization as dense batch sizes are chosen as multiple of $128$, which are hardware-friendly shapes for GEMM implementation without padding.} \pllm{} explores all possible kernel implementations varying the number of thread blocks, the number of warps, and tile size for GEMM, GEMV and Network kernels to identify the implementation that provides the shortest execution time. The profiling outputs a mapping from (kernel, batch size) to its best implementation with shortest execution time.

\textbf{Profiling kernels with interference}
However, when two or more kernels execute in parallel on a device, they slow down compared to running individually. We refer to this as \textit{kernel interference}, which is partially attributed to kernels competing for GPU hardware resources such as execution units, caches, and memory bandwidth. 

Understanding the interference characteristics by profiling overlapped kernels is challenging due to the large number of possible kernel combinations. Although each operation has only a few hundred kernel implementations, the combinations between different implementations of overlapping kernels exponentially expand the profiling space, resulting in millions of possible configurations. This immense complexity makes exhaustive exploration infeasible.




\pllm{} reduces the vast profiling space by selecting the thread block numbers for GEMV and network kernels from $8$ to $128$ (in steps of $8$) where kernel performance stabilizes around $128$. It also excludes less efficient GEMM kernels which have longer execution time with more thread blocks. It analyzes pairwise interferences of compute-memory and compute-network rather than combined kernel interference, focusing on compute-bound LLM serving to assess how other kernels impact compute performance.


\pllm{} profiles the selected GEMM-GEMV kernel pairs (\textasciitilde100 for A100 GPU) and sorts them by descending GEMM performance as in Figure \ref{fig:interference} (Network kernels are profiled similarly). For instance, a normalized performance of $0.8$ means the kernel’s execution time is $1/0.8$ times longer than the fastest implementation. Pairs with non-monotonic GEMV performance increase (grayed-out in Figure \ref{fig:interference}) are discarded, leaving the best-performing combinations at various GEMM-GEMV performance points.

 

\input{figure-tex/fig-gemm-gemv-interference}

\input{figure-tex/tab-occu}

Using interference profiles, \auto{} generates an \textit{interference table} (Table \ref{tab: occu}), which quantifies the performance of GEMV and network kernels as functions of interference on GEMM. For example, as depicted by the dotted red line in Figure \ref{fig:interference}, achieving $0.3$ GEMV performance requires sacrificing $0.2$ GEMM performance (from $1$ to $0.8$). This implies a non-linear trade-off: $0.2$ GEMM performance is exchanged for $0.3$ GEMV performance.


Through a sensitivity analysis of all GEMM shapes present in the models we evaluate (\S\ref{sec:evaluation}) and $16$ batch size combinations, we determine that interference results are similar with respect to those parameters (within a standard deviation of 5\% from the mean). 
\yilong{cannot understand this paragraph. add resource utilization definition here}

\subsubsection{\Auto{} Stage I: Pipeline Structure Search}
\label{subsec: pipeline-search}
In the first stage, \auto{} takes as input the dense batch size, the operation dependencies (defined in the PyTorch implementation of a given model architecture), and the profiling of kernel interferences, and then produces as output, the number, batch size, and order of each \nanoop{} using mixed integer linear programming (MILP). Stage I does not factor in the interference between \nanoop{}s to simplify the problem, which will be covered by Stage II. The MILP is subject to the constraints described below. 


\textbf{Optimization objective.} The main objective of the MILP is to remove pipeline bubbles (denoted by wasted in \fig{fig:exist-pipe}) for compute operations to minimize execution time.


\textbf{Constraints on the number of \nanoop{}s.} 
To overlap resources, every operation needs to be split into at least two \nanoop{}s, each operating on an independent \nano{}. Since splitting into \nanoop{}s reduces the batching effect, the number of \nanoop{}s should be minimized. Accordingly, \auto{} begins its search by dividing all operations into two \nanoop{}s. If the temporary best solution contains bubbles for compute, \auto{} increases the number of \nanoop{}s for operations near the bubble to improve resource utilization.
\gzuo{this step seems like greedy search, rather than modeled into MILP. Need rephrasing?}

\textbf{Constraints on batch sizes and durations.} \Auto{} forces the batch sizes to be chosen from $128$ to dense batch size and uses the interference-free duration of a \nanoop{} for a given batch size, as computed in \S\ref{subsec:kernel-profile}.



\textbf{Constraints on dependencies.}
The dependencies of \nanoop{}s are determined by their parent operations (present in the baseline architecture implementation) and the ranges of their batch sizes. \gzuo{nit: "range of batch sizes" confused me a bit. Maybe better: intersection/overlapping on their batch size dimension.} Two \nanoop{}s are dependent if and only if their parent operations are dependent (e.g., an O-projection depends on an attention operation) and their batch size ranges intersect (e.g., ranges 0–255 and 128–383). 

\textbf{Constraints on overlapping.}
Overlapping kernels constrained by the same resource (e.g., compute) is unhelpful for utilization, so \auto{} restricts the pipeline to overlap only operations constrained by different resources.

\textbf{Constraints on operation transformations.}
Some network collectives in LLM inference have equivalent transformations with different performance characteristics and dependencies. For example, an AG can be converted into an AR with different weight partitioning approaches~\cite{megatron-lm,alpa}. \pllm{} explores all of these alternative transformations for network \nanoop{}s.




 
\subsubsection{\Auto{} Stage II: Refining the Pipeline}
\label{subsec: resource-search}
\new{
The pipeline derived in the first stage does not factor in kernel interference, which is not practical.
In the second stage, \auto{} refines the pipeline from the prior stage by considering the kernel slowdown due to interference.
The second stage uses a separate MILP instance, where the numbers, batch sizes, and ordering constraints of \nanoop{}s remain the same as the output of the first stage. 
The \auto{} assigns resource utilization to individual \nanoop{}s, which affects the run time of \nanoop{}s, with the goal of minimizing pipeline execution time. Resource utilization ($R$) is defined as the normalized fraction of GPU resources (simultaneous multiprocessors) required to achieve a compute utilization of $R \times Compute$, where $Compute$ represents the GPU's peak compute capacity (\S\ref{sec:costfactors}). A specific resource utilization directly corresponds to kernel implementations as determined in \S\ref{subsec:kernel-profile}.\yilong{what is the resource utilization here? i guess is SM number. this is confusing}
}



\textbf{Constraints on GPU resource utilization.} While trying to minimize end-to-end execution time, \auto{} must assign kernels to \nanoop{}s, such that the collective normalized GPU resource utilization at any given time is less than or equal to 1 (i.e., 100\%). However, resource utilization of different kernels isn't directly fungible. For example, a GEMV kernel might achieve 0.3$\times$ of peak performance by only interfering with (reducing) 0.2$\times$ of peak GEMM performance as we show in Table~\ref{tab: occu}. Therefore, \auto{} consults the kernel interference profiling results when upholding the constraint that resource utilization is less than or equal to 1 at all times.

\textbf{Constrains on durations.} Given the resource utilization $\alpha$ for a \nanoop{} of a given type, \auto{} computes the duration of the operation using $D_{\text{best}} / \alpha$, where $D_{\text{best}}$ represents the best execution time without interference for the \nanoop{} given the \nano{} size, as determined by profiling (\S\ref{subsec:kernel-profile}).





\subsubsection{Example Pipelines}
\label{subsec: case-study}

\textbf{70B pipeline} We apply \auto{} to 70B-scale models, including \lm{}-2 70B, \lm{}-3 70B, Qwen2.5-72B, and Deepseek-67B. Compared to \lm{}-2 70B, \lm{}-3 70B features a larger vocabulary size of $128$K; Deepseek-67B has a slightly different number of layers and hidden dimension ($D_{model}$), Qwen2.5-72B introduces bias in KQV generation. However, none of these adjustments significantly change the performance characteristics, leading to similar schedules. We provide the \pllm{}-generated pipeline for \lm{}-2 70B as an example in \fig{fig:compute-pipe}.
\input{figure-tex/fig-compute-pipe}
\new{Since three resources (compute, memory, and network) overlap at the beginning of a decoding layer (i.e., KQV generations), \auto{} ends up using $4$ \nanoop{}s for this part, to reduce the pipeline bubbles. Here, the decode attention kernel has resource utilization $0.4$, i.e. reduces $40\%$ GEMM performance, which reaches 80\% of maximum decode attention performance. For the remainder of the pipeline, GEMM operations are prioritized, and only two \nanoop{}s are used. }

\textbf{8B pipeline} 8B models (e.g. Llama3-8B) do not require network operations as they fit in a single GPU. Thus \auto{} splits all operations into two \nanoop{}s, with decode attention overlapping with the UG and D operations.

\textbf{MoE pipeline} 
Compared to 70B models, MoE models have different hidden dimensions and number of layers. Due to the imbalance between experts\cite{mistral}, \pllm{} use tensor parallelism for MoEs, in which FFN is implemented using grouped-GEMM. FFN also involves an additional gate routing operation. 
\Auto{} works similarly for an MoE model and produces an efficient pipeline~(\S\ref{sec:evaluation}).



\subsection{Work in progress 4.1.1 version2: Profiling kernels with interference}
When two or more kernels execute in parallel on a device, they slow down compared to running individually. We refer to this as \textit{kernel interference}, which is attributed to kernels competing for GPU hardware resources such as execution units, caches, and memory bandwidth. To quantify this effect, we define Resource utilization (R) as a unified measurement of the GPU hardware resource consumed by each kernel. Interference is modeled by constraining the sum of resource utilization across all concurrent kernels to 100\%. The kernel performance under interference is then captured by the relationship between resource utilization (\(R\)) and performance (\(P\)), which is unique for different operations and must be determined through profiling.

However, directly profiling the relationship between $R$ and $P$ is infeasible as we cannot directly control the allocation of hardware units. 
Instead, we approximate this relationship by profiling the overlapping performance of kernels. 
Specifically, we empirically define the mapping of \(R\) to \(P\) for GEMM kernels: if a GEMM kernel achieves \(P_{\text{GEMM}}\%\) of peak performance when overlapped with another kernel, its resource utilization is defined as  \(R_{\text{GEMM}}=P_{\text{GEMM}}\).
The mappings for other kernels are then determined by measuring their normalized performance $P_{\text{other}}\%$. In the previous case, the other kernel consumes $R_{\text{other}} = 1-R_{\text{GEMM}}$, if the other kernel reaches $P_{\text{other}}\%$ of its peak performance, we conclude that $1-R_{\text{GEMM}}$ maps to $P_{\text{other}}$. 
Intuitively, we are exchanging $R_{\text{other}} =1-R_{\text{GEMM}}$ compute performance with $P_{\text{other}}$ memory or network kernel performance.
We define $R$ in a GEMM-centric way since the compute-bound operations dominate and optimizing compute is the goal of \pllm{}. 

Nonetheless, profiling the mapping between \(R\) and \(P\) remains challenging due to the vast number of possible kernel combinations.
While each operation may have only a few hundred kernel implementations, the combinations between different implementations of overlapping kernels exponentially expand the profiling space, resulting in millions of possible configurations.
This immense complexity makes exhaustive exploration infeasible.

\pllm{} reduces the vast profiling space by limiting the thread block numbers for GEMV and network kernels to values between \(8\) and \(128\) (in steps of \(8\)), as \(128\) is sufficient to saturate their performance.
It also excludes less efficient GEMM kernels which have longer execution times while using more thread blocks. 
\pllm{} also focuses on pairwise interference analysis---compute-memory and compute-network---rather than examining three kernel types simultaneously.

For GEMM shape \((M,N,K) = (384, 4096, 4096)\), GEMV batch size \(384\), and sequence length \(1024\), \pllm{} profiles approximately \(100\) GEMM-GEMV kernel pairs on the A100 GPU (Network kernels are profiled similarly). These pairs are then sorted by descending GEMM performance, as shown in Figure \ref{fig:interference}. 
For instance, a normalized performance of $0.8$ means the kernel’s execution time is $1/0.8$ times longer than the fastest implementation. 
Pairs with higher interference on GEMM but worse GEMV performance (grayed-out in Figure \ref{fig:interference}) are discarded. This process identifies the best-performing kernel combinations at various GEMM-GEMV performance trade-off points.

Using interference profiles, \auto{} generates an \textit{interference table} (Table \ref{tab: occu}). This table quantifies GEMV and network kernel performance as functions of GEMM interference, equivalent to the performance (\(P\)) of other kernels at a given resource utilization (\(R\)).
For example, as depicted by the dotted red line in Figure \ref{fig:interference}, achieving $0.3$ GEMV performance requires sacrificing $0.2$ GEMM performance (from $1$ to $0.8$). 
This implies a non-linear trade-off: $0.2$ GEMM performance is exchanged for $0.3$ GEMV performance, indicating that \(R_{\text{GEMV}} = 0.2\) corresponds to \(P_{\text{GEMV}} = 0.3\).


A sensitivity analysis of all GEMM shapes in the evaluated LLM models and 64 batch size combinations reveals that the \(R\) to \(P\) mapping is consistent, with a standard deviation within \(5\%\) of the mean.
Consequently, Table \ref{tab: occu} serves as the \(R\) to \(P\) mapping for all GEMV and network kernels in subsequent \auto{} analyses for simplicity.




